An Efficient Density-based Clustering Algorithm for Higher-Dimensional Data

DBSCAN is a typically used clustering algorithm due to its clustering ability for arbitrarily-shaped clusters and its robustness to outliers. Generally, the complexity of DBSCAN is O(n^2) in the worst case, and it practically becomes more severe in higher dimension. Grid-based DBSCAN is one of the recent improved algorithms aiming at facilitating efficiency. However, the performance of grid-based DBSCAN still suffers from two problems: neighbour explosion and redundancies in merging, which make the algorithms infeasible in high-dimensional space. In this paper, we propose a novel algorithm named GDPAM attempting to extend Grid-based DBSCAN to higher data dimension. In GDPAM, a bitmap indexing is utilized to manage non-empty grids so that the neighbour grid queries can be performed efficiently. Furthermore, we adopt an efficient union-find algorithm to maintain the clustering information in order to reduce redundancies in the merging. The experimental results on both real-world and synthetic datasets demonstrate that the proposed algorithm outperforms the state-of-the-art exact/approximate DBSCAN and suggests a good scalability.

==> alg+func.tex <==
% you should add these commands into the actionable-episode.tex file
\let\algorithm\relax
\let\endalgorithm\relax
\usepackage[linesnumbered,vlined,ruled]{algorithm2e} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5

\begin{figure}[!t]
\linesnumbered \SetVline
\begin{algorithm}[H]
\caption{Basic Maintenance Approach}\label{alg:basicF}
\KwIn{$\alpha$: a frequent minimal-occurrence episode\; \\

$ET_{\alpha}$: the set of end time of each MEO of $\alpha$\;\\
$\epsilon$: the threshold of maximum window size for consequent occurrence\;  \\
$\mathit{min}\_\mathit{freq}$: minimum frequency threshold generating a valid PER\; }
\KwOut{$\mathcal{T}_{\alpha}$: the complete ARE-trie w.r.t antecedent $\alpha$\;}
\SetVline
\Begin{
build a root node $r$ of $\mathcal{T}_{\alpha}$ where $r$.$\mathit{episode}$$\gets$$\alpha$ and $r$.$\mathit{tlist}$$\gets$ $ET_{\alpha}$\;
$\mathrm{ExtendNode}$$($$r$, $\epsilon$, $\mathit{min}\_\mathit{freq}$$)$\;
}
\end{algorithm}

\begin{function}[H]\nonumber
\linesnumbered \dontprintsemicolon
\caption{ExtendNode($q$)}
\SetVline
\KwIn{$q$: node to be extended\; \\
$\epsilon$: the threshold of maximum window size for consequent occurrence\;  \\
$\mathit{min}\_\mathit{freq}$: minimum frequency threshold generating a valid PER\; }
\KwOut{$\mathcal{T}_{\alpha}$: updated PER-trie w.r.t antecedent $\alpha$\;}
\SetVline
\Begin{
    $d$ $\gets$ distance between the root node $r$ and $q$\;
    \For{$i$$=$$1$ to $(\epsilon - d)$}{
        $\mathit{position}\_\mathit{List}$ $\gets$ $\{$$t'~|~t'=t+i, t \in q.\mathit{tlist}$$\}$\;\label{alg:extend-l3}
        scan $\vec{S}$ on each time stamp in $\mathit{position}\_\mathit{List}$ and get an event set $E'$ such that the frequency of every event in $E'$ is not less than $\mathit{min}\_\mathit{freq}$\;\label{alg:extend-l4}
        \ForEach{$e' \in E'$\label{alg:extend-l5}}{
            $q'$.$\mathit{event}$ $\gets$ $e'$\;
            $Q$ $\gets$ the set of occurrence times of $e'$ in $\mathit{position}\_\mathit{List}$\;\label{alg:extend-l7}
             $q'$.$\mathit{tlist}$ $\gets$ $Q$\;
            put $q'$ as the child of $q$\;\label{alg:extend-l8}
            $\mathrm{ExtendNode}$$($$q', \epsilon, \mathit{min}\_\mathit{freq}$$)$\;\label{alg:extend-l9}
        }
    }
    }
\end{function}
\end{figure}
